Denoising based Sequence-to-Sequence Pre-training for Text Generation

This paper presents a new sequence-to-sequence (seq2seq) pre-training method PoDA (Pre-training of Denoising Autoencoders), which learns representations suitable for text generation tasks. Unlike encoder-only (e.g., BERT) or decoder-only (e.g., OpenAI GPT) pre-training approaches, PoDA jointly pre-trains both the encoder and decoder by denoising the noise-corrupted text, and it also has the advantage of keeping the network architecture unchanged in the subsequent fine-tuning stage. Meanwhile, we design a hybrid model of Transformer and pointer-generator networks as the backbone architecture for PoDA. We conduct experiments on two text generation tasks: abstractive summarization, and grammatical error correction. Results on four datasets show that PoDA can improve model performance over strong baselines without using any task-specific techniques and significantly speed up convergence.

==> Makefile <==
# 被编译的主文件的文件名，不包括扩展名。
JOBNAME = emnlp-ijcnlp-2019
# 这个变量的值可以为 latex、pdflatex 或 xelatex。
LATEX = xelatex
BIBTEX = bibtex
DVIPDF = dvipdfmx

# 如果用 LaTeX 编译，则使用 dvipdfmx 将 dvi 转成 pdf。
ifeq ($(LATEX), latex)
	DODVIPDF = $(DVIPDF) $(JOBNAME)
endif

MAKE = make
RM = rm -f

all:
	$(LATEX) $(JOBNAME)
	$(BIBTEX) $(JOBNAME)
	$(LATEX) $(JOBNAME)
	$(LATEX) $(JOBNAME)
	$(DODVIPDF)

.PHONY: clean dist-clean
clean:
	$(RM) $(JOBNAME).log $(JOBNAME).aux $(JOBNAME).out  $(JOBNAME).thm\
		$(JOBNAME).toc $(JOBNAME).lof $(JOBNAME).lot $(JOBNAME).blg\
		$(JOBNAME).bbl $(JOBNAME).dvi missfont.log $(JOBNAME).synctex.gz
	$(RM) chap/*.aux

dist-clean: clean
	$(RM) $(JOBNAME).pdf

